Multi-Scale Verification of Distributed Synchronisation

Algorithms for the synchronisation of clocks across networks are both common and important within distributed systems. We here address not only the formal modelling of these algorithms, but also the formal verification of their behaviour. Of particular importance is the strong link between the very different levels of abstraction at which the algorithms may be verified. Our contribution is primarily the formalisation of this connection between individual models and population-based models, and the subsequent verification that is then possible. While the technique is applicable across a range of synchronisation algorithms, we particularly focus on the synchronisation of (biologically-inspired) pulse-coupled oscillators, a widely used approach in practical distributed systems. For this application domain, different levels of abstraction are crucial: models based on the behaviour of an individual process are able to capture the details of distinguished nodes in possibly heterogenous networks, where each node may exhibit different behaviour. On the other hand, collective models assume homogeneous sets of processes, and allow the behaviour of the network to be analysed at the global level. System-wide parameters may be easily adjusted, for example environmental factors inhibiting the reliability of the shared communication medium. This work provides a formal bridge across the abstraction gap separating the individual models and the population-based models for this important class of synchronisation algorithms.

==> figo.tex <==



\iffalse

\section{Formal Verification and Probabilistic Model Checking}
\mwcomment{Section taken from FiGo verification paper.. need to update}

Formal methods are a family of techniques used to verify software and
hardware, typically using mathematical, proof-based
approaches~\cite{fisher11introduction}. These include techniques such
as automated theorem proving~\cite{fitting96first}, in which full
mathematical proof is carried out, and model
checking~\cite{Baier2008}, in which every state of a model (also known
as the model's \emph{state space}) can be examined
exhaustively. Formal methods allow for \emph{formal verification},
where models of software and hardware systems can be proved to satisfy
certain requirements. These requirements are typically provided using
a precise formal logical language such as temporal
logic~\cite{fisher11introduction}. In this paper we use
\emph{probabilistic} model-checking~\cite{Kwiatkowska2011}, a variant
of traditional model-checking that allows for probabilities to be
incorporated into a model, and for quantitative analyses to be carried
out on such models. In traditional model checking the result of formal
verification is a Boolean value indicating whether or not a model
satisfies the prescribed property; by contrast, probabilistic model
checking allow us to find the probability that a particular model satisfies
that property. Probabilistic model checking is essential for capturing
and analyzing the stochastic nature of WSN, e.g., communication
errors, or changes in ambient temperature resulting in clock
drift. Additionally, the \emph{quantitative} nature of probabilistic
model checking allows it to be used for performance evaluation based
on the time elapsed or energy consumed, for
example~\cite{KNP09a,Haverkort:2005:PV:1059816.1059817,Baier:2005:MCM:1059816.1059819,Kwiatkowska:2005:PMC:1059816.1059820}.
%\subsection{Formal Verification}


\subsection{The \prism{} Model Checker}

\lstset{language=Pseudocode,basicstyle=\sffamily,tabsize=2,numbers=left,columns=flexible}

%A formal model of the FiGo algorithm shown in Figure~\ref{f:figo} was
%created using \prism{}~\cite{Kwiatkowska2011,prism-manual}. 
In this paper we use the probabilistic model checker, \prism{}~\cite{Kwiatkowska2011,prism-manual}. \prism{} consists of two parts: a modeling language, and a model checker. The
\prism{} modeling language can be used to specify the behaviour of a
\emph{probabilistic} finite state automaton (P-FSA), which can then be
formally verified via the model checker.  For
example, a sensor node that can either transmit a message or remain
idle can simply be modelled using a P-FSA as follows:
%\ednote{FSA here}
%\begin{center}
%\includegraphics[scale=0.8]{pstricks/fsm-crop.pdf}
%\end{center}
%We can add transitions, if we wish, to denote that the light switch can remain on or off.
%\begin{center}
%\includegraphics[scale=0.8]{pstricks/fsm1-crop.pdf}
%\end{center}
%We can also label the edges of this automaton with probabilities:
\begin{center}
\includegraphics[scale=0.8]{figures/fsm2-crop.pdf}
\end{center}
The two states, `transmit' and `idle', are linked with arrows, or
transitions. These transitions specify how the state of the P-FSA can
change. The annotations on the transitions show the probability that
the transition will be taken. In this case there is a probability of
0.99 that the sensor remains in its current state, and a probability
of 0.01 that the state will change. Note that these values can either
be chosen arbitrarily, or with reference to a particular practical
sensor implementation. For example, a specific sensor may spend more
time transmitting than idling, in which case the probabilities
associated with these transitions can be modified.
%\begin{center}
%\includegraphics[scale=0.8]{pstricks/fsm3-crop.pdf}
%\end{center}



%Finite state automata with probabilities are known as probabilistic finite state automata. 
The \prism{} language can be used to specify several variants of P-FSAs,
including discrete-time Markov chains (DTMCs), continuous-time Markov
chains (CTMCs) as well as Markov decision pro\-cess\-es~(MDPs)~\cite{prism-manual}. In this paper we use only DTMCs.

We can model the sensor node above in the \prism{} modelling language
as follows:
\begin{verbnobox}[\sffamily\small]
module sensorNode
   state: [0..1] init 0;Just spoke to Sven and he said you are going to 
   [] state=0 -> 0.99: (state'=0) + 0.01: (state'=1);
   [] state=1 -> 0.99: (state'=1) + 0.01: (state'=0);	
endmodule
\end{verbnobox}

\noindent This sensor node is modelled as a module in \prism{}. We have
one variable, `state', which can be set to 0 or 1 (which we define as
representing `transmit' and `idle' respectively). Note that we define an
initial state of 0 for this variable. There are two lines denoting
commands. The first command says that if the state is 0, then remain
in state 0 with probability 0.99 or transition to state 1 with
probability 0.01. The second command is similar, but with 0 and 1
reversed. In general, commands take the form
$$
\mathsf{[s]}\ \mathsf{guard}\ \textsf{->}\ \mathsf{p_1: u_1} + \ldots + \mathsf{p_n: u_n ;}
$$ 
%
where $\mathsf{p_i}$ are probabilities and $\mathsf{u_i}$ are lists of
variable updates. In the case where only one list of updates is made
with probability 1.0, a simpler form is used (e.g.,
$\mathsf{[s]}\ \mathsf{guard}\ \textsf{->}\ \mathsf{u;}$).  The letter
$\mathsf{s}$ denotes an optional synchronization. Synchronized
commands execute simultaneously with synchronization commands from
other modules that share the same label, and can be used for
inter-module communication. Another way for modules to communicate is
via the use of \emph{local variables}, which can be read by all
modules, as well as \emph{gJust spoke to Sven and he said you are going to lobal variables} which can be read by, and
written to, all modules.

Multiple modules can be specified within a \prism{} model. Models are
executed by selecting non-deterministically a command (from any
module) whose guard evaluates to true. If there are no commands whose
guards are true, then the model has reached a fixed point and will
stop executing.


Once a formal model has been developed in the \prism{} language, it can be formally verified, with respect to some requirement, using the \prism{} model checker. \prism{} requirements can be formalized as \emph{properties} using logical languages such as probabilistic computation tree logic (PCTL) and probabilistic linear temporal logic (P--LTL)~\cite{Baier2008}. Different logics allow different kinds of properties to be specified. In this paper we will use PCTL to specify properties. 

PCTL is based on a discrete formulation of time as a tree-like structure, starting from a particular point and extending into the future. The following are valid PCTL formulae:
%\begin{itemize}
 `$p$', meaning that $p$ is true;
 `$\neg p$', meaning that $p$ is false;
 `$p \implies q$', meaning if $p$ is true then $q$ is true; 
 $p\wedge q$', meaning that both $p$ and $q$ are true;
 `$\eventually{p}$', meaning $p$ is true now or at some point in the future; and
 `$\always{p}$', meaning $p$ is true now and at every point in the future. %\ednote{tidy}
%\end{itemize}
\prism{} also allows the use of standard numerical operators such as $=$, $\ge$ and $\le$.

Formal verification works by analyzing the entire state space of a model in order to determine whether a particular property holds. For example, for the sensor node model above, we can use PCTL to specify that the sensor node is eventually in the `idle' state:
$$
\eventually(\var{state}=1) 
$$
This can then be turned into a property in \prism{} by adding the $P^{=?}[\ldots]$ operator around the PCTL formula. This operator indicates that we are querying \prism{} for the probability of the formula being true on some path through the model:
$$
P^{=?} [\eventually(\var{state}=1) ] = 1.0
$$Just spoke to Sven and he said you are going to 
In this case, \prism{} has determined that the probability is 1.0. More complex properties can be formed. For example, the following property gives the probability that the model will always be in the `idle' state at some point:
$$
P^{=?} [\always\eventually(\var{state}=1) ] = 1.0
$$
This kind of property is said to specify the probability that the model is in the `idle' state \emph{infintely often}. 
%We can also use \prism{} to verify that the \prism{} model is a correct representation of the probabilistic FSA shown earlier. For example, we can determine the probability of the model being in the idle state immediately after being in the `transmit' state:



%\ednote{TODO: show basic properties}

\fi
  

\section{The Firefly-Gossip (FiGo) Protocol}
\mwcomment{Section taken from FiGo verification paper.. need to update}

Current techniques for large-scale computer management are not
suitable for WSN due to the unreliable nature of the nodes and their
networks. A potential solution is to use management protocols, such as FiGo, that
 scale well and are robust to the failure of individual nodes.  In
applications such as precision
agriculture~\cite{abbasi2014review,ojha2015wireless}, wireless nodes
need to be synchronized to be able to deliver time-correlated samples
of data such as moisture levels and temperature, and to analyze the
data. If the analysis shows a problem, control messages need to be
sent to nodes with actuators, e.g., to increase irrigation in a
drought, or decrease it if a particular disease is discovered.

Synchronization of a WSN isJust spoke to Sven and he said you are going to  essential in many applications, for
example in adaptive sensing for smart water
networks~\cite{kartakis2016adaptive}.  WSN allow urban water
providers to monitor the water flow to match customer demand.
Synchronization enables the sensor nodes to measure, communicate and
aggregate the flow rates and water pressure data. A control algorithm
on the actuator nodes can open or close valves to stabilize water flow
for the network, or re-route water in the case of a major
leak. Importantly, the control software can also disseminate new
control algorithms or critical security updates to all the sensing and
actuation nodes via gossiping. 

%In this paper we show the applicability of formal verification for
%performance evaluation of WSN. To demonstrate this, we focus on the
%correctness of a decentralized WSN management protocol,
%Firefly--Gossip, or FiGo~\cite{breza2008lessons}. 
FiGo is typical of a
class of algorithms that combine firefly
synchronization~\cite{wernerallen2005fis} and gossip
protocols~\cite{jelasity2005gba} into a single epidemic process~\cite{breza2008lessons}. This
mixture of synchronization and dissemination processes is used to
bring the internal states of WSN nodes to a stable, global equilibrium
where all nodes are synchronized with respect to both time and
metadata. Experiments have shown such protocols to be both scalable
and resilient to individual node
failure~\cite{breza2008lessons,breza13phd,breza2017polite}. A typical
FiGo algorithm is shown in Figure~\ref{f:figo}.
Just spoke to Sven and he said you are going to 
\begin{figure}[tb]
 \centering
 \small
 \includegraphics[width=.8\columnwidth]{figures/figocode2.pdf}
 \caption{Phases of the FiGo Gossip--Synchronization Algorithm.}
  \label{f:figo}
\end{figure}

% Do we need this paragraph???
%FiGo was developed first as a software application within a laboratory setting, and was evaluated experimentally.
%In addition, the TOSSIM simulator \cite{levis2003taa} was used with code written in NesC
%\cite{gay2003nlh} for the TinyOS operating system. Populations of up to 100
%nodes were simulated, and the protocol was observed to function. The
%simulations confirmed that the ideas behind FiGo were sound. Simulation
%results were limited by the difficulty of accurately modelling radio
%communication. To complement the simulation efforts the Figo algorithm was also evaluated through remote execution on 77 sensor nodes at the Motelab
%\cite{wernerallen2005mws} test bed at Harvard University, and on 117 sensor nodes at the  Indriya
%\cite{doddavenkatappa2012indriya} test bed at the National University of Singapore. These experiments 
%confirmed that the  FiGo algorithm can be 
%deployed on a real radio network subject to real-world radio communication
%problems like unreliability and interference. It did, however have a limited,
%fixed topology, and so our evaluation was limited to the topological
%constraints of the test bed. It is conceivable that certain topologies would
%cause problems for FiGo.

FiGo algorithms have been deployed for the synchronization and management of
several WSN deployments run by the Adaptive Emergent Systems
Engineering group at Imperial
College\footnote{http://wp.doc.ic.ac.uk/aese/}. For example, they were
used to organize pollution sensors for an experiment with mobile data
mules as part of an Imperial College Grand Challenge project, and to
synchronize and control the sampling rate for a rainfall monitoring
sensor network as part of a floodplain monitoring project done in
collaboration with the Imperial College Department of Civil
Engineering. They are currently undergoing evaluation for 
deployment across the Liverpool Sensor City IoT-X/LoRaWAN
network\footnote{http://www.sensorcity.co.uk/}.



%\section{Firefly--Gossip (FiGo) Protocols}



%\section{Modelling Protocols in \prism{}}

\subsection{A \prism{} Model of FiGo}

A \prism{} model of FiGo was developed precisely capturing the control
flow of the algorithm in Figure~\ref{f:figo}. The algorithm begins
with a number of variable assignments which are directly translated
into variable assignments in \prism{}. Some of the variables are not
updated at all in the model, so these are set as global constants in
\prism{}, e.g.:
\begin{verbnobox}[\sffamily\small]
const int cycleLength = 100;
const int refractoryPeriod = floor(cycleLength/2);  	
\end{verbnobox}
The main loop of the algorithm is then divided into a number of
phases. For example, the \texttts{transmit} phase corresponds to the
if-statement in lines 9 to 14. The next
if-statement consists of a number of nested if-statements called
\texttts{listen}, \texttts{sync1}, \texttts{sync2}, and so on. The
final phase corresponds to the final if-statement in the main loop and
is called \texttts{updateClock}. These phases are defined as global
constants and were used as the values of a local variable
\texttts{s1Phase} which contains the currently-executing phase:
\begin{verbnobox}[\sffamily\small]
 s1Phase : [0..9] init transmit;
\end{verbnobox}
Note that \texttts{s1Phase} refers to the phase of the first sensor
node module, which is called \texttts{s1}. Other sensor node modules
are called \texttts{s2}, \texttts{s3}, etc.

When one phase has finished executing the next phase is chosen
according to the control flow of the algorithm in
Figure~\ref{f:figo}. For example, during the \texttts{sync1} phase in lines 16
to 18 the algorithm checks whether a message has been overheard (i.e., received), and if the clock is outside the refractory period. 
If they are, then the sensor updates its clock to the average of its own clock and the clock of the other sensor. The ``circular average'' is used, in which the average of 90 and 10 are 0 (modulo 100), rather than 50. The circular average ensures that the update to the clock variable moves it closer to the clock of the other sensor.

In the \prism{}
model, this behaviour is shown in the following three commands:
\begin{verbnobox}[\sffamily\small]
[] s1Phase=sync1 & s1LocalClock>=refractoryPeriod & 
  diff<=floor(cycleLength/2) -> 
  (s1LocalClock'=s1avg1) & (s1Phase'=sync2);
[] s1Phase=sync1 & s1LocalClock>=refractoryPeriod & 
  diff>floor(cycleLength/2) -> 
  (s1LocalClock'=s1avg2) & (s1Phase'=sync2);
[] s1Phase=sync1 & !( s1LocalClock>=refractoryPeriod ) 
  -> (s1Phase'=sync2); \end{verbnobox}
The first two commands say that if the sensor is in the \texttts{sync1}
phase and the clock is greater than or equal to \texttts{refractoryPeriod}, then set \texttts{s1}'s clock to the circular average of the \texttts{s1}'s clock and \texttts{s2}'s clock. The third command says that if these conditions aren't set, then proceed to the next phase of the algorithm, \texttts{sync2}.


%The FiGo algorithm is asynchronous: sensors broadcast a message and continue executing without waiting to see if any other sensors have received the message, i.e., message broadcast is non-blocking. 
%The command then updates the phase to \texttts{updateClock}, which
%causes the sensor to increment the clock.  The second command says
%that if the phase is \texttts{transmit} and the conditions on the
%clock and the \texttts{sameCount} are not satisfied, then no messages
%are sent and the phase is updated to \texttts{clockCycleCheck}, which
%is the next phase of the algorithm seen in line 16.
The sensor which we have modelled here is called \texttts{s1}. To
model communication between sensor nodes we need at least one more
sensor in the model, \texttts{s2}. The sensor \texttts{s2} is exactly
the same as \texttts{s1}, except all references to ``\texttts{s1}'' in
the code are modified to ``\texttts{s2}.'' 
Communication in the model is achieved
asynchronously through the use of inboxes: when a sensor sends a
message to another sensor it does so by leaving the message in an
inbox, which can then be read by the receiving sensor when it is ready
to do so.

The resulting combined
model is around 140 lines of code long including variable
declarations, and can be found online\footnote{To appear in the final
  version of the paper.}. This \prism{} model is an almost direct
translation from the pseudocode to \prism{} and has not been optimized
for formal verification.


==> figures/figocode/mylistings.tex <==
\newcounter{lst}[section]

\renewcommand{\thelst}{\arabic{section}.\arabic{lst}}

\lstdefinestyle{easslisting}{basicstyle=\footnotesize\sffamily, mathescape=true, frame=tb,  numbers=right, numberstyle=\footnotesize, stepnumber=1, numbersep=-5pt, captionpos=b}


\lstdefinestyle{listingl}{basicstyle=\footnotesize\sffamily, mathescape=true, numberstyle=\footnotesize, stepnumber=1, numbersep=-5pt, captionpos=b}

\lstdefinestyle{eass}{basicstyle=\sffamily, mathescape=true}

\lstnewenvironment{listing}[3]{
  \noindent        
  \refstepcounter{lst}         
  \label{code:#1}  
\begin{tabular}{p{.97\columnwidth}} \\ \hline  {\normalsize \textbf{Code  fragment \arabic{section}.\arabic{lst}} #2} \\  \end{tabular} 
\lstset{language=#3,          
  basicstyle=\footnotesize\sffamily,
%%%  basicstyle=\footnotesize,    
  xleftmargin=10pt,    
  mathescape=true,    
  frame=tb,    
  numbers=right,    
%%%  numberstyle=\tiny,     
  numberstyle=\footnotesize,     
  stepnumber=1,     
  numbersep=-5pt}}{}

  
%-- definition for Pseudocode --%

\lstdefinelanguage{Pseudocode}{%
    morekeywords={mod,or,and,if,end,then,else,loop,while},
    morecomment=[l]{//},
 literate= {<-}{{$\leftarrow$}{$\:$}}2
           {.B}{{${\cal B}$}}2
           {.G}{{${\cal G}$}}2
           {lnot}{{$\sim$}}2
           {varr}{{$R$}}2
           {varn}{{$n$}}2
           {varc}{{$T$}}2
           {funf}{{$\Delta$}}2           
           {varclock}{{$\Phi$}}2
           {coupling}{{$\epsilon$}}2
           {assert_shared}{{$+_{\Sigma}$}}2
           {remove_shared}{{$-_{\Sigma}$}}2
           {True}{{$\top$}}2
           {(perform)}{}0
}

  
  
%-- definition for Gwendolen --%

\lstdefinelanguage{Gwendolen}{%
    morekeywords={Plans,Initial,Beliefs,Goals,name,fof-parse,Rules,Belief},
    morecomment=[l]{//},
 literate= {<-}{{$\leftarrow$}{$\:$}}2
           {.B}{{${\cal B}$}}2
           {.G}{{${\cal G}$}}2
           {lnot}{{$\sim$}}2
           {assert_shared}{{$+_{\Sigma}$}}2
           {remove_shared}{{$-_{\Sigma}$}}2
           {True}{{$\top$}}2
           {(perform)}{}0
}




==> notation.tex <==

\section{Notation}
\label{sec:notation}

Let \(f\colon A \to B\) be a function. We use the notation
\(\override{f}{x}{y}\) to express \emph{updating \(f\) at \(x\) by \(y\)}. 
That is, the function that coincides with \(f\), except for \(x\), where it 
takes the value \(y\). 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sync_journal"
%%% End: 

==> pco.tex <==
\section{Pulse-Coupled Oscillators and Network Synchronisation}






%Note that the abstraction gap between concrete models and the algorithms themselves is much less significant, as the concrete models closely resemble the algorithms on which they are based~\cite{figopaper}.

